ShortcutLens: A Visual Analytics Approach for Exploring Shortcuts in Natural Language Understanding Dataset

Benchmark datasets play an important role in evaluating Natural Language Understanding (NLU) models. However, shortcuts -- unwanted biases in the benchmark datasets -- can damage the effectiveness of benchmark datasets in revealing models' real capabilities. Since shortcuts vary in coverage, productivity, and semantic meaning, it is challenging for NLU experts to systematically understand and avoid them when creating benchmark datasets. In this paper, we develop a visual analytics system, ShortcutLens, to help NLU experts explore shortcuts in NLU benchmark datasets. The system allows users to conduct multi-level exploration of shortcuts. Specifically, Statistics View helps users grasp the statistics such as coverage and productivity of shortcuts in the benchmark dataset. Template View employs hierarchical and interpretable templates to summarize different types of shortcuts. Instance View allows users to check the corresponding instances covered by the shortcuts. We conduct case studies and expert interviews to evaluate the effectiveness and usability of the system. The results demonstrate that ShortcutLens supports users in gaining a better understanding of benchmark dataset issues through shortcuts, inspiring them to create challenging and pertinent benchmark datasets.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> source_tex/5-methods.tex <==
\section{Methods}
% This section is to introduce some methods we proposed. How you mine the templates.
In this section, we first introduce the algorithm used to find potential shortcuts from \mzhihua{benchmark datasets}. 
\mzhihua{Then we introduce how shortcuts are grouped and summarized for better understanding. }
Finally, we propose a what-if analysis method that allows users to estimate the improvements after removing selected shortcuts. 

% We are going to introduce the core methods used in the system including template mining, aggregation, and what if analysis.
\begin{figure}[htb]
\centering 
\includegraphics[width=\linewidth]{figs/ShortcutMethods.pdf}
\caption{Methods. } 
\label{Fig.methods}
\end{figure}

\subsection{Shortcut Mining}

%% 1. How we mine the template?
% \zhihua{Current terms seem confuse the template, rule, and the shortcuts.}
% \zhihua{The motivation behind the template mining, aggregation, and what if analysis seems unclear.}

To help extract the potential shortcuts in the dataset, it is desirable to have a suite of algorithms to mine the potential shortcuts from the \mzhihua{benchmark dataset.} 
We first assume that the potential shortcuts are matching-based shortcuts, that is, if the text contains the specific pattern, it will be considered covered by these potential shortcuts. 
Inspired by the defined shortcuts in DQI~\cite{mishra2020dqi} and the structural templates which include Part-of-Speech (POS) and \mzhihua{named entities} from Tempura~\cite{wu2020tempura}, we define the pattern as a set of spatially-related words. 
Specifically, we consider one word with its POS, or two words with their POS and their relative position (\ie, how many words are in between) to define the pattern or template. For example, we consider one pattern as follows: (1) The first word \dq{The} is a determiner. (2) The second word \dq{will} is a verb. (3) The first word is in front of the second word, and there is a word between them. Such a pattern can match sentences such as \dq{The men will all leave.}
The components of the potential shortcuts can be abbreviated, that is, some components of it can be optional appearing in the potential shortcuts. For example, in the template above, the scope of the second word can be extended by considering this word as a verb, and not just the specific word \dq{will}. The newly defined template is the parent of the original template.
The mining algorithm selects shortcuts with high \textit{productivity} and \textit{coverage}~\cite{niven2019probing,branco2021shortcutted}.
Coverage refers to the number of instances covered by the shortcut. The prediction label of the potential shortcut is defined as the dominant label in the label distribution. Productivity is calculated as the percentage of covered instances with the same label as the prediction label in covered instances. 


The basic idea of the mining algorithm is extracting potential shortcuts via an exhaustive method. Then it will filter potential shortcuts based on the productivity and coverage. Finally, it will organize the shortcuts into a hierarchical structure. The details are illustrated as follows: % The potential shortcuts mining algorithm works as follows: 
\begin{itemize}
    \item[(1)] 
    Once we have the POS and words for a specific text, we will enumerate each word in the text to determine the POS of the first word and then its specific word.
    \item[(2)] 
    We will enumerate the possible relative position to get the position of the next word and its specific POS and word. % From this path, we have four potential shortcuts. [First POS], [First POS, First word], [First POS, First word, Relative Position, Second POS], [First POS, First word, Relative Position, Second POS, Second Word],
    \item[(3)] 
    The label distribution for each potential shortcut will be updated accordingly. If the specific instance has been considered in the specific potential shortcut, we will only consider that the potential shortcut covers that instance only once.
    \item[(4)]
    We will calculate the coverage and productivity for each potential shortcut.
    \item[(5)]
    We will filter the potential shortcuts by a preset minimum coverage and productivity in the whole set. Also, we will consider the minimum coverage and productivity in each set, like the training set, development set, and test set.
    \item[(6)]
    After getting a set of filtered potential shortcuts, we will organize the filtered potential shortcuts into a hierarchical structure based on the definition of the parent relationship.
    \item[(7)]
    To reveal the relationship between the filtered potential shortcuts, we will track the paths from the root of the hierarchy of the potential shortcuts to filtered potential shortcuts and the children of filtered potential shortcuts.
\end{itemize}




\subsection{Shortcut Aggregation}

After running the shortcut mining algorithm, we find that there are a large number of potential shortcuts in the \mzhihua{benchmark dataset.} One of the reasons is that the number of different words is quite large. It imposes difficulty for users to explore such large-scale potential shortcuts. Therefore, we aggregate similar potential shortcuts based on the semantic meaning of the words to reduce the difficulty for users to explore. 


%% 1. Why we need template aggregation?
% Since the number of the tokens under the same kind of part-of-speech is large, we adopt similarity-based hierarchical clustering technique to aggregate the similar templates. 

%% 2. How do we employ techniques to implement the aggregation?


The basic idea of the shortcut aggregation algorithm is using hierarchical clustering to aggregate potential shortcuts with similar words based on word embedding into a new shortcut and insert this shortcut into the original hierarchy of shortcuts. The details are illustrated as follows: 
%The basic idea of shortcut aggregation algorithm is 
%The potential shortcuts aggregation algorithm runs as follows. 
\begin{itemize}
    \item[(1)]
    We first check whether the two potential shortcuts can be merged, and then we calculate the distances between every two potential shortcuts. If two potential shortcuts share the same parent, the same prediction label, and the final component of each potential shortcut is the word, we will calculate the distances for the two final words. The distance between two final words $ftok$ is defined as $1-Sim(ftok_{a}, ftok_{b})$. The similarity between two words $Sim$ is defined as the cosine similarity of word embeddings for those two words. Then the distances between two potential shortcuts will be set to the distances between two final words. If two potential shortcuts do not satisfy the conditions for merging, the distances between these two potential shortcuts will be set to infinity.
    \item[(2)]
    We adopt hierarchical clustering with complete linkage to cluster similar potential shortcuts based on the distances between two potential shortcuts~\cite{clusterAnalysis}. 
    \mzhihua{We have empirically set the clustering methods as the complete linkage as we found that such a method can ensure that the distance between each shortcut will be under a certain threshold, which is empirically set as 0.75.}
    \item[(3)] 
    If a cluster of potential shortcuts has more than one potential shortcut, it will be converted into a new potential shortcut, and this new potential shortcut will be inserted into the hierarchy of the potential shortcuts. Concretely, the parent of this new potential shortcut is set to the parent of the potential shortcuts in this cluster. Then the parent of the potential shortcuts in this cluster will be updated to this new potential shortcut. The children of this new potential shortcut and the parent of this new potential shortcut will be updated accordingly. The final word of this new potential shortcut is defined as the final word of potential shortcuts with the smallest average distances to all other final words in the same cluster. This new potential shortcut covers the instances covered by all potential shortcuts in that cluster. For the meaning of this new potential shortcut, it means that if the text contains the words specified by the set of final words in the cluster in the specific position, it will be considered that this new potential shortcut covers that instance. 
    % Then this centroid is the representative of this potential shortcut. 
    % \item[(3)]
    % We will update the hierarchical relationship between the potential shortcuts. The children of this new potential shortcut will be set to the potential shortcuts in the cluster. The parent of this new potential shortcut is set to the potential shortcut with the longest prefix without considering the final word. For the meaning of this new potential shortcut, it means that if the text contains the words specified by the set of final words in the cluster in the specific position, it will be considered that this new potential shortcut covers that instance. 

\end{itemize}


\subsection{What-If Analysis}

In order to help dataset creators decide which potential shortcuts should be fixed and what actions should be taken to fix the potential shortcuts, a what-if analysis on shortcuts of interest is necessary for dataset creators to make decisions. Possible actions can be taken to fix potential shortcuts in the same \mzhihua{benchmark dataset.} They include constructing new instances, modifying the existing instances, or removing the existing instances to battle against a group of potential shortcuts. Dataset creators can also compose a set of actions to fix the potential shortcuts. However, after taking action, it is hard for dataset creators to know whether it really resolve the issues. Therefore, a necessary what-if analysis should be considered. We will take an initial attempt to consider the influence of the removal of a group of instances.


%% 1. What is the definition of dirty set and clean set?
After users have focused on a group of shortcuts of interest, the instances covered by these shortcuts will be found. We will consider the instances covered by them as the dirty set and the instances not covered by them as the clean set. 
\mzhihua{There are a few differences} in calculating productivity between a group of potential shortcuts and one potential shortcut. 
When calculating the productivity for a group of potential shortcuts, it is possible that one instance is covered by multiple potential shortcuts with different prediction labels. Those instances will be considered as \dq{disagreed} instances. The number of \dq{disagreed} instances will be calculated. Then, the productivity for a group of shortcuts will be defined as the percentage of covered \dq{agreed} instances with the same prediction label as the corresponding potential shortcuts. Such metrics indicate the impact of those potential shortcuts.

If machine prediction results are provided by users, we will calculate the machine accuracy for the dirty set and clean set respectively. It is interesting to compare the machine accuracy between the whole set and the clean set to see whether the removal of potential shortcuts will lead to degrading performance metrics in the clean set. Such indicators can help dataset creators understand the potential benefits gained from the removal of the instances covered by those potential shortcuts.


